Particle Gibbs Split-Merge Sampling for Bayesian Inference in Mixture Models

This paper presents a new Markov chain Monte Carlo method to sample from the posterior distribution of conjugate mixture models. This algorithm relies on a flexible split-merge procedure built using the particle Gibbs sampler. Contrary to available split-merge procedures, the resulting so-called Particle Gibbs Split-Merge sampler does not require the computation of a complex acceptance ratio, is simple to implement using existing sequential Monte Carlo libraries and can be parallelized. We investigate its performance experimentally on synthetic problems as well as on geolocation and cancer genomics data. In all these examples, the particle Gibbs split-merge sampler outperforms state-of-the-art split-merge methods by up to an order of magnitude for a fixed computational complexity.

==> notation.tex <==
%%%% WARNING: CURRENTLY ONLY USED BY REBUTTAL FILES (STUFF COPIED INTO MAIN LATEX FILE)



\usepackage{notation}

% conventions:
%  vector:             [letter]Vec   eg: \sigmaVec
%  split-merge subset: [letter]Bar   eg: \sBar

% these are needed to override some of the existing macros later on
\let\rawpi\pi
\let\rawsigma\sigma
\let\rawphi\phi
\let\rawgamma\gamma
\let\rawtau\tau
\let\rawtheta\theta

% indices
\notation*[Index of a block (cluster)]{k}{k}
\notation*[Observation index]{i}{i}
\notation[Particle index]{p}{p}
\notation[Number of particles used in the particle Gibbs algorithms]{N}{N}
\notation*[SMC generation (iteration) index]{t}{t}
\notation[Number of points to allocate, also coincides with the number of particle Gibbs generations (iterations)]{n}{n}

% main notation used in the paper:
\notation*[Bijection from particles to restricted clusterings]{phi}{\rawphi}
\notation[Proposal distribution for the particle Gibbs algorithm]{q}{q}
\notation*[Intermediate un-normalized distributions]{gamma}{\rawgamma}
\notation[Number of datapoints]{T}{T}
\notation*[One block in a clustering]{b}{b}
\notation[All observations]{yVec}{\bold{y}}
\notation[One observed datapoint]{y}{y}
\notation*[Partition or clustering of the observation indices]{c}{c}
\notation[Subset of observation indices; in particular, set of anchor points]{s}{s}
\notation*[Parameter of the parametric family]{theta}{\rawtheta}
\notation*[Likelihood of the parametric family]{L}{L}
\notation*[Prior for the parametric family, and base measure of the process]{H}{H}
\notation*[Prior over clusterings]{tau}{\rawtau}
\notation*[Target density of interest]{pi}{\rawpi}
\notation[Factor in the clustering prior depending on the number of clusters]{tauI}{\protect{\rawtau_1}}
\notation[Factor in the clustering prior depending on the size of each block]{tauII}{\protect{\rawtau_2}}
\notation[Closure of a subset of datapoint indices relative to a clustering]{sBar}{\overline{s}}
\notation[Restriction of the clustering to the closure subset]{cBar}{\overline{c}}
\notation[Split merge target distribution]{piBar}{\overline{\rawpi}}
\notation[Split merge modification of the prior factor depending on the number of clusters]{tauIBar}{\overline{\rawtau}_1}
\notation[A binary relationship indicating whether two datapoint indices are in the same block (relative to some clustering specified as a subscript)]{isclusteredwith}{\sim}
\notation[A support restriction on the split merge target]{I}{I}
\notation[Blocks of the partition outside of the closure]{cMinus}{c_{-}}
\notation[Auxiliary target distribution]{piTilde}{\tilde{\rawpi}}
\notation[Distribution of the anchors]{h}{h}
\notation[Markov kernel used to conceptualized a whole split-merge step]{K}{K}
\notation[Permutation auxiliary variable vector]{sigmaVec}{\boldsymbol{\rawsigma}}
\notation*[Permutation auxiliary variable component]{sigma}{\rawsigma}
\notation[Allocation decision (a particle is made of a vector of such allocations)]{x}{x}
\notation[State space containing the possible allocation decisions]{X}{\mathcal{X}}
\notation[Particle]{xVec}{\bold{x}}
\notation[Support defining valid sequences of allocation decisions]{partSupport}{\mathcal{S}}
\notation[Resampling ancestry variable]{ancestor}{a}
\notation[Resampling ancestry vector]{ancestors}{\boldsymbol{a}}
\notation*[Conditional resampling distribution]{r}{r}
\notation[Weight variable]{w}{w}
\notation[Weight vector]{wVec}{\boldsymbol{w}}
\notation[Markov kernel used to conceptualized a particle Gibbs step]{KBar}{\overline{K}}
\notation[Particle Gibbs auxiliary variables]{g}{g} 
\notation[Annealing schedule used to delay the introduction of the clustering prior]{schedule}{\zeta}
\notation[Sufficient statistics for the likelihood]{suffstat}{\psi}
\notation{nclust}{\protect{|c|}}
\notation[Relative ESS threshold used for adaptive resampling]{ressThreshold}{\beta}

% Hyperparameters of the examples of clustering priors
\notation[Concentration parameter used in clustering priors such as the Dirichlet process]{concentration}{\protect{\alpha_0}}
\notation[Discount parameter used in the Pitman-Yor process]{discount}{d}
\notation[Maximum number of clusters in the finite Dirichlet model]{maxnclust}{\k_0}
\notation[Symmetric concentration parameters for the finite Dirichlet model]{finiteconcentration}{\alpha_{\textrm{Dir}}}




==> tex/basic-math-macros.tex <==
\newcommand\labelledmapsto[1]{\stackrel{#1}{\longmapsto}}



\usepackage{array}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{mathtools}
\newcommand\defeq{\coloneqq}

\DeclareMathOperator{\expd}{Expd}
\DeclareMathOperator{\support}{support}

\newcommand\priorprior{q_{\textrm{pr-pr}}}
\newcommand\wpriorprior{w_{\textrm{pr-pr}}}

\newcommand\priorpost{q_{\textrm{pr-po}}}
\newcommand\wpriorpost{w_{\textrm{pr-po}}}

\newcommand\unrootedclades{\Sigma_\textrm{u}}
\newcommand\rootedclades{\Sigma_\textrm{r}}

\newcommand\rootedbl{b_\textrm{r}}
\newcommand\unrootedbl{b_\textrm{u}}

\newcommand\pmmetric{d_\textrm{PM}}
\newcommand\rfmetric{d_\textrm{L1}}
\newcommand\kfmetric{d_\textrm{L2}}

\newcommand\bracearray[1]{\left\{ \begin{array}{l} #1 \end{array} \right.}
\newcommand\bracearraypair[2]{\bracearray{#1 \\ #2}}
\newcommand\bracearraytriple[3]{\bracearray{#1 \\ #2 \\ #3}}
\newcommand\bracearrayquad[4]{\bracearray{#1 \\ #2 \\ #3 \\ #4}}
\newcommand\dotprod[2]{\langle #1, #2\rangle}

\newcommand\tspaceum{\tspace_\textrm{um}}
\newcommand\tspacenc{\tspace_\textrm{nc}}

\newcommand\parname[1]{\noindent{\bf #1}}

\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}


\newcommand\observations{\mathcal Y}
\newcommand\poset{\mathcal S}
\newcommand\sigmaalg{{\mathcal F}}

\newcommand\bracearraycond[1]{\left\{ \begin{array}{ll} #1 \end{array} \right.}

\newcommand\partialderiv{\frac{\partial}{\partial \theta_i}}

\def\Q{{\mathbb Q}}        % rationals
\def\Z{{\mathbb Z}}        % integers
\def\NN{{\mathbb N}}        % naturals
\def\RR{{\mathbb R}}        % reals

\def\P{{\mathbb P}}        % probability
\def\E{{\mathbb E}}        % expectation 
\def\1{{\mathbf 1}}        % indicator
\def\var{{\mathop{\mathbf Var}}}    % variance


\def\ascv{\stackrel{\scriptscriptstyle a.s.}{\longrightarrow}}     % almost sure convergnece
\def\pcv{\stackrel{\scriptscriptstyle \P}{\longrightarrow}}        % convergence in P
\def\ltcv{\stackrel{\scriptscriptstyle\L^2}{\longrightarrow}}      % L2 convergnece
\def\lpcv{\stackrel{\scriptscriptstyle\L^p}{\longrightarrow}}      % Lp convergnece
\def\dcv{\stackrel{\scriptscriptstyle d}{\longrightarrow}}         % convergence in d
\def\deq{\stackrel{\scriptscriptstyle d}{=}}         % equal in d
\def\iidsim{\stackrel{\scriptscriptstyle \textrm{iid}}{\sim}}         % iid
\def\toinf{\to \infty}

\def\ci{\perp\!\!\!\perp}  % conditional independence

\DeclareMathOperator{\parent}{pa}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


\newcommand\transp[1]{{#1}^{\textrm{T}}}


\newcommand{\ud}{\,\mathrm{d}}

\newcommand\aX{{\cal X}}
\newcommand{\apath}{{\mathbf s}}



\DeclareMathOperator{\dom}{dom}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}




==> tex/typesetting-macros.tex <==
\usepackage{textcomp,mathrsfs}
\usepackage{graphicx,amssymb,amsmath,amsthm,mathrsfs}
\usepackage{multirow,makeidx} %,algorithmic,algorithm}
\usepackage{latexsym,graphicx,amssymb,amsmath,amsthm,mathrsfs}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{booktabs,fancyhdr} 
\usepackage{url}
\usepackage{vmargin}
\usepackage{hyperref}

\setmarginsrb{2cm}{2cm}{2cm}{3cm}{0cm}{0cm}{0cm}{1cm}

% This gives you control over how far down in the hierarchy the
% table of contents will print.
\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}
 
\usepackage{url}
%%%%% URL package fix %%%%%
\begingroup
\makeatletter
\g@addto@macro{\UrlSpecials}{%
  \endlinechar=13 \catcode\endlinechar=12
  \do\%{\Url@percent}\do\^^M{\break}}
 \catcode13=12 %
 \gdef\Url@percent{\@ifnextchar^^M{\@gobble}{\mathbin{\mathchar`\%}}}%
\endgroup %

\makeindex 

\graphicspath{{./graphics/},{./figures/}}

\newcounter{xxx}
\setcounter{xxx}{0}
\newcommand\XXX[1]{{\bf [[TODO \#\addtocounter{xxx}{1}\thexxx: #1]]}}

% For rebuttal:

\newcommand{\comment}[1]{\noindent\textbf{Comment:} \emph{#1}}


